Automatic dysarthric speech detection exploiting pairwise distance-based convolutional neural networks

Automatic dysarthric speech detection can provide reliable and cost-effective computer-aided tools to assist the clinical diagnosis and management of dysarthria. In this paper we propose a novel automatic dysarthric speech detection approach based on analyses of pairwise distance matrices using convolutional neural networks (CNNs). We represent utterances through articulatory posteriors and consider pairs of phonetically-balanced representations, with one representation from a healthy speaker (i.e., the reference representation) and the other representation from the test speaker (i.e., test representation). Given such pairs of reference and test representations, features are first extracted using a feature extraction front-end, a frame-level distance matrix is computed, and the obtained distance matrix is considered as an image by a CNN-based binary classifier. The feature extraction, distance matrix computation, and CNN-based classifier are jointly optimized in an end-to-end framework. Experimental results on two databases of healthy and dysarthric speakers for different languages and pathologies show that the proposed approach yields a high dysarthric speech detection performance, outperforming other CNN-based baseline approaches.

==> tikz/AF_HR.tex <==
% This file was created by tikzplotlib v0.9.1.
\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
\begin{tikzpicture}

\begin{axis}[
%colorbar,
%colorbar style={width=0.2cm, xshift=-0.1cm, ylabel style = {yshift=0.45cm, xshift = 0.25cm}, ylabel={\scriptsize \begin{tabular}{c}Normalized \\amplitude)\end{tabular}}},
colormap={mymap}{[1pt],
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta max=3.69,
point meta min=-1.62,
tick align=outside,
tick pos=left,
%title={Healthy STFT},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=57.5,
%xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=57.5,
ytick style={color=black},
 width = 0.47*\linewidth, 
height = 0.22*\textwidth,
ylabel style = {yshift=-0.4cm, xshift = -0cm},
xlabel style = {yshift=0.18cm, xshift = -0cm},
xlabel= {\scriptsize \begin{tabular}{c}Time frame from\\ a reference representation\end{tabular}},
ylabel={\scriptsize \begin{tabular}{c}Time frame from a test \\ dysarthric representation\end{tabular}},
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=57.5, ymin=-0.5, ymax=57.5] {tikz/AF_PR.png};
\end{axis}

\end{tikzpicture}


%
%
%% This file was created by matplotlib2tikz v0.7.5.
%\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
%\begin{tikzpicture}
%\begin{axis}[
%%colormap default colorspace=rgb,
%colorbar,
%colorbar style={width=0.2cm, xshift=-0.1cm, ylabel style = {yshift=0.45cm, xshift = 0.25cm}, ylabel={\scriptsize \begin{tabular}{c}Power/frequency \\(dB/$\frac{1}{3}$octave)\end{tabular}}},
%colormap={mymap}{[1pt]
%  rgb(0pt)=(0,0,0.5);
%  rgb(22pt)=(0,0,1);
%  rgb(25pt)=(0,0,1);
%  rgb(68pt)=(0,0.86,1);
%  rgb(70pt)=(0,0.9,0.967741935483871);
%  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
%  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
%  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
%  rgb(132pt)=(1,0.925925925925926,0);
%  rgb(178pt)=(1,0.0740740740740741,0);
%  rgb(182pt)=(0.909090909090909,0,0);
%  rgb(200pt)=(0.5,0,0)
%},
%point meta max=22,
%point meta min=-30,
%tick align=outside,
%tick pos=left,
%x grid style={white!69.01960784313725!black},
%xlabel={Time frame index},
%xmin=-0.5, xmax=35.5,
%xtick style={color=black},
%y grid style={white!69.01960784313725!black},
%%ylabel={Octave band},
%ymin=-0.5, ymax=14.5,
%ytick style={color=black},
% width = 0.45*\linewidth, 
%height = 0.25*\textwidth,
%]
%%\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5] {octavecontrol-000.png};
%
%\addplot+[shader=flat] graphics [xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5, includegraphics] {tikz_figs/octave/octavecontrol-000-cutted2.png};
%%sharp plot 
%\end{axis}
%
%\end{tikzpicture}


==> tikz/AF_PR.tex <==
% This file was created by tikzplotlib v0.9.1.
\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
\begin{tikzpicture}
\begin{axis}[
colorbar,
colorbar style={width=0.15cm, xshift=-0.25cm, ylabel style = {yshift=-1.9cm, xshift = -0cm}, ylabel={\scriptsize \begin{tabular}{c}distance value\\ (globally normalized)\end{tabular}}},
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta max=3.69,
point meta min=-1.62,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=57.5,
%xtick style={color=black},
%xtick={-10,0,10,20,30,40,50,60},
%xticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,},
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=57.5,
%ytick style={color=black},
%ytick={-10,0,10,20,30,40,50,60},
%yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,},
 width = 0.45*\linewidth, 
height = 0.22*\textwidth,
ylabel style = {yshift=-0.4cm, xshift = -0cm},
xlabel style = {yshift=0.18cm, xshift = -0cm},
xlabel= {\scriptsize \begin{tabular}{c}Time frame from\\ a reference representation\end{tabular}},
ylabel={\scriptsize \begin{tabular}{c}Time frame from a test \\ healthy representation\end{tabular}},
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=57.5, ymin=-0.5, ymax=57.5] {tikz/AF_HR.png};
\end{axis}

\end{tikzpicture}



%
%
%% This file was created by matplotlib2tikz v0.7.5.
%\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
%\begin{tikzpicture}
%\begin{axis}[
%%colormap default colorspace=rgb,
%colorbar,
%colorbar style={width=0.2cm, xshift=-0.1cm, ylabel style = {yshift=0.45cm, xshift = 0.25cm}, ylabel={\scriptsize \begin{tabular}{c}Power/frequency \\(dB/$\frac{1}{3}$octave)\end{tabular}}},
%colormap={mymap}{[1pt]
%  rgb(0pt)=(0,0,0.5);
%  rgb(22pt)=(0,0,1);
%  rgb(25pt)=(0,0,1);
%  rgb(68pt)=(0,0.86,1);
%  rgb(70pt)=(0,0.9,0.967741935483871);
%  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
%  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
%  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
%  rgb(132pt)=(1,0.925925925925926,0);
%  rgb(178pt)=(1,0.0740740740740741,0);
%  rgb(182pt)=(0.909090909090909,0,0);
%  rgb(200pt)=(0.5,0,0)
%},
%point meta max=22,
%point meta min=-30,
%tick align=outside,
%tick pos=left,
%x grid style={white!69.01960784313725!black},
%xlabel={Time frame index},
%xmin=-0.5, xmax=35.5,
%xtick style={color=black},
%y grid style={white!69.01960784313725!black},
%%ylabel={Octave band},
%ymin=-0.5, ymax=14.5,
%ytick style={color=black},
% width = 0.45*\linewidth, 
%height = 0.25*\textwidth,
%]
%%\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5] {octavecontrol-000.png};
%
%\addplot+[shader=flat] graphics [xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5, includegraphics] {tikz_figs/octave/octavecontrol-000-cutted2.png};
%%sharp plot 
%\end{axis}
%
%\end{tikzpicture}


==> tikz/HR.tex <==
% This file was created by tikzplotlib v0.9.1.
\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
\begin{tikzpicture}

\begin{axis}[
%colorbar,
%colorbar style={width=0.2cm, xshift=-0.1cm, ylabel style = {yshift=0.45cm, xshift = 0.25cm}, ylabel={\scriptsize \begin{tabular}{c}Normalized \\amplitude)\end{tabular}}},
colormap={mymap}{[1pt],
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta max=2,
point meta min=-1.2,
tick align=outside,
tick pos=left,
%title={Healthy STFT},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=57.5,
%xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=57.5,
ytick style={color=black},
 width = 0.47*\linewidth, 
height = 0.22*\textwidth,
ylabel style = {yshift=-0.4cm, xshift = -0cm},
xlabel style = {yshift=0.18cm, xshift = -0cm},
xlabel= {\scriptsize \begin{tabular}{c}Time frame from\\ a reference template\end{tabular}},
ylabel={\scriptsize \begin{tabular}{c}Time frame from\\ a test dysarthric template\end{tabular}},
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=57.5, ymin=-0.5, ymax=57.5] {tikz/PR.png};
\end{axis}

\end{tikzpicture}


%
%
%% This file was created by matplotlib2tikz v0.7.5.
%\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
%\begin{tikzpicture}
%\begin{axis}[
%%colormap default colorspace=rgb,
%colorbar,
%colorbar style={width=0.2cm, xshift=-0.1cm, ylabel style = {yshift=0.45cm, xshift = 0.25cm}, ylabel={\scriptsize \begin{tabular}{c}Power/frequency \\(dB/$\frac{1}{3}$octave)\end{tabular}}},
%colormap={mymap}{[1pt]
%  rgb(0pt)=(0,0,0.5);
%  rgb(22pt)=(0,0,1);
%  rgb(25pt)=(0,0,1);
%  rgb(68pt)=(0,0.86,1);
%  rgb(70pt)=(0,0.9,0.967741935483871);
%  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
%  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
%  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
%  rgb(132pt)=(1,0.925925925925926,0);
%  rgb(178pt)=(1,0.0740740740740741,0);
%  rgb(182pt)=(0.909090909090909,0,0);
%  rgb(200pt)=(0.5,0,0)
%},
%point meta max=22,
%point meta min=-30,
%tick align=outside,
%tick pos=left,
%x grid style={white!69.01960784313725!black},
%xlabel={Time frame index},
%xmin=-0.5, xmax=35.5,
%xtick style={color=black},
%y grid style={white!69.01960784313725!black},
%%ylabel={Octave band},
%ymin=-0.5, ymax=14.5,
%ytick style={color=black},
% width = 0.45*\linewidth, 
%height = 0.25*\textwidth,
%]
%%\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5] {octavecontrol-000.png};
%
%\addplot+[shader=flat] graphics [xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5, includegraphics] {tikz_figs/octave/octavecontrol-000-cutted2.png};
%%sharp plot 
%\end{axis}
%
%\end{tikzpicture}


==> tikz/PR.tex <==
% This file was created by tikzplotlib v0.9.1.
\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
\begin{tikzpicture}
\begin{axis}[
colorbar,
colorbar style={width=0.15cm, xshift=-0.25cm, ylabel style = {yshift=-1.9cm, xshift = -0cm}, ylabel={\scriptsize \begin{tabular}{c}distance value\\ (globally normalized)\end{tabular}}},
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta max=2,
point meta min=-1.2,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=57.5,
%xtick style={color=black},
%xtick={-10,0,10,20,30,40,50,60},
%xticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,},
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=57.5,
%ytick style={color=black},
%ytick={-10,0,10,20,30,40,50,60},
%yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,},
 width = 0.45*\linewidth, 
height = 0.22*\textwidth,
ylabel style = {yshift=-0.4cm, xshift = -0cm},
xlabel style = {yshift=0.18cm, xshift = -0cm},
xlabel= {\scriptsize \begin{tabular}{c}Time frame from\\ a reference template\end{tabular}},
ylabel={\scriptsize \begin{tabular}{c}Time frame from\\ a test healthy template\end{tabular}},
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=57.5, ymin=-0.5, ymax=57.5] {tikz/HR.png};
\end{axis}

\end{tikzpicture}



%
%
%% This file was created by matplotlib2tikz v0.7.5.
%\tikzset{ font={\fontsize{7pt}{7}\selectfont}}
%\begin{tikzpicture}
%\begin{axis}[
%%colormap default colorspace=rgb,
%colorbar,
%colorbar style={width=0.2cm, xshift=-0.1cm, ylabel style = {yshift=0.45cm, xshift = 0.25cm}, ylabel={\scriptsize \begin{tabular}{c}Power/frequency \\(dB/$\frac{1}{3}$octave)\end{tabular}}},
%colormap={mymap}{[1pt]
%  rgb(0pt)=(0,0,0.5);
%  rgb(22pt)=(0,0,1);
%  rgb(25pt)=(0,0,1);
%  rgb(68pt)=(0,0.86,1);
%  rgb(70pt)=(0,0.9,0.967741935483871);
%  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
%  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
%  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
%  rgb(132pt)=(1,0.925925925925926,0);
%  rgb(178pt)=(1,0.0740740740740741,0);
%  rgb(182pt)=(0.909090909090909,0,0);
%  rgb(200pt)=(0.5,0,0)
%},
%point meta max=22,
%point meta min=-30,
%tick align=outside,
%tick pos=left,
%x grid style={white!69.01960784313725!black},
%xlabel={Time frame index},
%xmin=-0.5, xmax=35.5,
%xtick style={color=black},
%y grid style={white!69.01960784313725!black},
%%ylabel={Octave band},
%ymin=-0.5, ymax=14.5,
%ytick style={color=black},
% width = 0.45*\linewidth, 
%height = 0.25*\textwidth,
%]
%%\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5] {octavecontrol-000.png};
%
%\addplot+[shader=flat] graphics [xmin=-0.5, xmax=35.5, ymin=-0.5, ymax=14.5, includegraphics] {tikz_figs/octave/octavecontrol-000-cutted2.png};
%%sharp plot 
%\end{axis}
%
%\end{tikzpicture}


==> tikz/grid.tex <==
%\tdplotsetmaincoords{60}{125}
\begin{tikzpicture}
    [tdplot_main_coords,
        grid/.style={very thin,blue}]

\foreach \x in {-2.5,-2,...,2.5}
    \foreach \y in {-2.5,-2,...,2.5}
    {
        \draw[grid] (\x,-2.5) -- (\x,2.5);
        \draw[grid] (-2.5,\y) -- (2.5,\y);
    }
\end{tikzpicture}
